Denoising Multi-Source Weak Supervision for Neural Text Classification

We study the problem of learning neural text classifiers without using any labeled data, but only easy-to-provide rules as multiple weak supervision sources. This problem is challenging because rule-induced weak labels are often noisy and incomplete. To address these two challenges, we design a label denoiser, which estimates the source reliability using a conditional soft attention mechanism and then reduces label noise by aggregating rule-annotated weak labels. The denoised pseudo labels then supervise a neural classifier to predicts soft labels for unmatched samples, which address the rule coverage issue. We evaluate our model on five benchmarks for sentiment, topic, and relation classifications. The results show that our model outperforms state-of-the-art weakly-supervised and semi-supervised methods consistently, and achieves comparable performance with fully-supervised methods even without any labeled data. Our code can be found at https://github.com/weakrules/Denoise-multi-weak-sources.

==> 1-intro.tex <==
\section{Introduction}

\zc{
Title: need to be more concrete, something like "Denoising Multi-Source Weak Supervision for Neural Text Classification" will probably be better

Introduction:

Paragraph 1: many NLP tasks can be formulated as text classification $\rightarrow$ dnns are successful $\rightarrow$ but they require labeled data, which are expensive to obtain $\rightarrow$ recently, pre-trained language models can alleviate this problem, but still suffers degraded performance when labeled data is limited.
\wendi{BERT still need labeled data}

Paragraph 2: weak supervision is promising, but also challenging to apply because weak labels are inaccurate and incomplete.

Paragraph 3: we study using multiple weak supervision sources to learn text classifiers; the intuition is multiple weak supervision sources can provide complementary information to eliminate noise; and combined with unlabeled data, they can address label incompleteness as well.
\wendi{key: complementary information; bootstrapping on D_U}

Paragraph 4: there are a large body of works on weakly-supervised learning, most are dealing with only single-source weak supervision $\rightarrow$ they may suffer from the unreliability of single sources and error propagation;
\wendi{sensitive to single source}
several works deal with multiple sources, but they XXX (for example, snorkel only do label denoising as a pre-processing step, not dealing with label incompleteness; simple majority voting is suboptimal because xxx; 
\wendi{snorkel: not with later classifier train} 
I believe there are other works on learning from multiple supervision sources (even not for text classification), need to make sure we cite and discuss them).

Paragraph 5: introduce our method, the key idea, the uniqueness compared with existing methods. I feel the current method description is a bit plain, need to distill the main ideas.
I think the main ideas are:
- source reliability estimation and neural classification benefit each other $\rightarrow$ the co-training framework 
\wendi{regularization}
- conditional source reliability
- self-training to leverage unmatched samples to obtain more labeled instances.
- maybe also mention we rely on pre-trained language models to get good representations, which helps denoising 
\wendi{high level: denoise, and how to enhance}

Other Sections:
Section 2: make it at most half a page
Section 3: 2.5 pages
Section 4: 3 pages
others: 1 page

Something we had better show in the experiments:
- multi-source weak supervision can be powerful (compared to existing single-source, fully supervised methods) $\rightarrow$ for this, we already have a lot of results
- majority voting does not work
- our method works better than existing weak supervision methods (make sure we include important baselines that also handle multiple weak supervision sources)
- what happens if we use some subsets of the multiple weak supervision sources
- are there any interpretations about the source reliability we learned
- how the different designs in our method work (corresponding to the main strategies we claimed in the introduction)
- would labeled data help further
}

Text classification, relation extraction, question answering are the fundamental natural language tasks with numerous
applications such as document classification or knowledge extraction. 
\zc{$\rightarrow$ Many NLP tasks can be formulated as text classification
  problems, such as sentiment analysis, topic classification, relation
  extraction, and XXX (maybe come up with another example from QA/Dialogue).}
Recently, deep neural nets (DNNs) have demonstrated superior performance for
this problem \zc{briefly mention earlier dnns (rnn, cnn), to the recent trend of
BERT-based ones}, largely due to their capabilities of automatically learning distributed features and fitting complex functions based on large-scale training data.  
However, in many real world scenarios, large-scale labeled data are unavailable
and manually annotating data at a large scale is prohibitively expensive.
\zc{merge paragraph 1 and 2}

To address the label scarcity bottleneck, we study the problem of  using
heuristic rules to train neural text classifiers.  While domain experts \zc{not
  necessarily domain experts, can be also KBs.} often cannot afford to annotate millions of documents carefully, they can easily provide a set of heuristic rules as weak supervision signals.  Using such rules can automatically induce labeled data for model training
\citep{ratner2017snorkel}, but meanwhile it introduces two major challenges:
\emph{label noise} and \emph{low label coverage}.
%The first challenge is \emph{label noise}. 

The \emph{label noise} issue arises because heuristic rules are often too simple to capture the rich contexts and complex patterns for text classification. For instance, while a rule `expensive \(\rightarrow\) negative' for restaurant ranking is correct for most times, but sometimes it wrong because the delicious food deserves the high price. Seed rules have \emph{limited coverage} because real-life text corpora often have
long-tail distributions, many heuristic rules are defined over the most
frequent keywords, so the instances containing only long-tail keywords cannot be covered by any given rules.
\zc{can merge the previous paragraph and shorten it.}

There have been studies \citep{ratner2017snorkel, meng2018weakly} that attempt to use weak supervision for deep text classification. Unfortunately, their performance is limited by the above two challenges. Ratner \etal
\citep{ratner2017snorkel} proposed a data programming method, which uses
heuristic rules as labeling functions and then trains discriminative models
using the automatically created labeled data. However, the training data
annotated by data programming come from instances that can be directly matched by the rules, making the model have limited performance on the unmatched data. 
Meng \etal \citep{meng2018weakly} proposed a deep self-training method, which uses weak supervision to learn an initial model and then updates the model by using the model's own confident predictions. However, the self-training procedure can overfit the label noise and suffer from the error propagation.

\sep \textbf{Our contributions.} We propose a new method that uses weak
supervision to train deep text classifiers in a label-efficient way, while
addressing the label noise and label coverage issues. We assume multiple weak
supervision sources (\eg, domain experts, knowledge bases) provide complementary
sets of heuristic rules. \zc{the previous two sentences can be merged.}
Our idea is that the complementary information in the multiple sources can not
only reduce label noise, but also effectively bootstrap on unlabeled data to
improve label coverage, making it possible to learn an accurate deep text
classifier with weak supervision. 

Motivated by the above, we propose a model with two carefully designed
components. The first component is a rule-based classifier \zc{$\rightarrow$ rule reliability estimators} using the conditional soft attention mechanism. Given weak labels from annotators and document representations, we learn reliability scores for labeling sources, which emphasize the weak annotators' opinions that are most informative for our particular corpus.
We then use the reliability scores to aggregate our disparate weak labels into a denoised pseudo label.
\zc{need to highlight that our rule reliability is conditional on input text features}

The second component is a neural classifier that learns labels and distributed feature representations for all samples, matched and unmatched. This neural classifier is supervised by both the denoised labels and its own confident predictions on the unmatched data, enabling it to solve the rule coverage problem while simultaneously enhancing the rule denoiser via patterns present in the unmatched data. 
The two components are integrated into a end-to-end training framework.

\zc{maybe we should also say we use pre-trained BERT as our feature extractor:
  its representation power can help our denoiser work better.}

We evaluate our model on four text classification tasks, including sentiment
analysis, topic classification, spam classification, and information
extraction. The results on five benchmarks show that: (1) the soft-attention module can indeed
effectively denoise the noisy training data induced from weak supervision
sources, achieving \textasciitilde{}$86$\% accuracy for denoising; and (2) the
co-training design can improve prediction accuracy for unmatched samples,
achieving at least $9$\% accuracy increase on them. In terms of the overall
performance, our model consistently outperforms state-of-the-art weakly
supervised methods \cite{ratner2017snorkel,meng2018weakly,zamani2018neural}, semi-supervised
methods \cite{tang2015pte}, and fine-tuning methods \cite{howard2018universal}
 by 9.2\% on average. Further, we show that the denoised labels can be fed into fully supervised models and fine-tune the models to improve their performance.


% Our contributions are summarized as follows:
% \begin{itemize}

%   \item We propose a neural co-training framework that leverages multi-source
%     weak supervision for deep text classification. The co-training design
%     jointly models multiple weak supervision sources to learn a text classifier
%     in an end-to-end manner. Such a co-training framework makes it possible to
%     learn accurate deep text classifiers without any labeled data.

%   \item We propose a label denoising module that can reduce label noise in weak
%     supervision. Based on a conditional soft attention mechanism to encode both data information and source knowledge, the denoising module
%     estimates source reliability to remove label noise effectively.  In
%     addition, we propose a self-trainable neural classifier, which tackles the
%     label coverage issue by bootstrapping on unlabeled data.
%     %\chao{emphasize conditional}

% \item We perform extensive experiments on five different benchmarks for four
%   text classification tasks. The results demonstrate our model outperforms
%   strong baselines, and achieves comparable performance to fully supervised
%   models without using any labeled data.

% \end{itemize}




%  ===============================================
% \textbf{Chao: I outline a structure for the intro, fill and extend these paragraphs!}

% % Paragraph 1: Text classification is one of the most fundamental problems in text mining, information retrieval, and natural language processing. While deep neural nets
% % have achieved dominant performance for text classification, they are highly label-hungry, often requiring hundreds of thousands of labeled samples to achieve strong performance.  This has become a key bottleneck of applying deep
% % text classifiers to many real-life applications, where large-scale labeled data are too expensive to obtain.

% % Paragraph 2: An overview of existing methods for handling label sparsity. Including: 
% % self-training methods,
% % fine-tuning methods, 
% % weakly supervised methods. Think hard about their drawbacks.

% % Paragraph 3: An overview of our model: we propose a deep neural text classifier, which is learned not from excessive labeled data, but only unlabeled data plus a set of easy-to-provide heuristic rules.

% % Paragraph 4: Two challenges of learning from rules: Learning the model from heuristic rules is difficult, because the rules can only induce noisy training data and can have limited coverage.

% % Paragraph 5: How we address the two challenges:
% % First, it has a label denoising module, which estimates source reliability and denoises rule-induced supervision with a soft attention mechanism. Second, it has a self-learning module for improving the label coverage issue, which iteratively predicts soft labels for unmatched samples by aggregating the denoised multi-source classifiers. The two modules are integrated into a neural co-training model, which can be learned in an end-to-end manner.

% % Paragraph 6: The results we obtain on real data

% % A bullet list summarizing our contributions:
